Matching Models for Graph Retrieval

Graph Retrieval has witnessed continued interest and progress in the past few years. In thisreport, we focus on neural network based approaches for Graph matching and retrieving similargraphs from a corpus of graphs. We explore methods which can soft predict the similaritybetween two graphs. Later, we gauge the power of a particular baseline (Shortest Path Kernel)and try to model it in our product graph random walks setting while making it more generalised.

==> background/background.tex <==
\chapter{Background}

==> conclusion/conclusion.tex <==
\chapter{Conclusion}

==> evaluation/evaluation.tex <==
\chapter{Evaluation}

==> project/tables.tex <==
\chapter{tables}

% Arre tables beech mein daalni h
% jaise SP_approach mein
% and trainable walks vale chapter mein
